A Continuous Relaxation for Discrete Bayesian Optimization

To optimize efficiently over discrete data and with only few available target observations is a challenge in Bayesian optimization. We propose a continuous relaxation of the objective function and show that inference and optimization can be computationally tractable. We consider in particular the optimization domain where very few observations and strict budgets exist; motivated by optimizing protein sequences for expensive to evaluate bio-chemical properties. The advantages of our approach are two-fold: the problem is treated in the continuous setting, and available prior knowledge over sequences can be incorporated directly. More specifically, we utilize available and learned distributions over the problem domain for a weighting of the Hellinger distance which yields a covariance function. We show that the resulting acquisition function can be optimized with both continuous or discrete optimization algorithms and empirically assess our method on two bio-chemical sequence optimization tasks.

==> preamble.tex <==
% preamble.tex
% Author: Michael Schober (michael.schober@tuebingen.mpg.de)
% Date: 2013/01/17
% LAST CHANGED: R.Michael, S.Bartels 2024/04/26

\usepackage{ifthen}

\RequirePackage{ifluatex}
\ifthenelse{\boolean{luatex}}
{
}
{
	% I'm using UTF-8 on this computer
	\usepackage[utf8]{inputenc} 
	\usepackage[T1]{fontenc} 
}

\usepackage{placeins} % for the command \FloatBarrier
\usepackage{flafter} % don't let figures appear before they are defined

% COLOR DEFINITIONS %%%%%%%%%%%
\usepackage{xcolor}
\definecolor{lred}{RGB}{200,0,0}
\definecolor{dred}{HTML}{7B332F} % PN red
\definecolor{dre}{HTML}{7B332F} % PN red
\definecolor{dblu}{HTML}{003e7d} % ETH blue
\definecolor{blu}{HTML}{003e7d} % ETH blue
\definecolor{lblu}{RGB}{125,125,255}
\definecolor{lgr}{RGB}{50,200,157}
\definecolor{lgre}{RGB}{50,200,157}
\definecolor{dgra}{RGB}{50,50,50}
\definecolor{mgra}{RGB}{100,100,100}
\definecolor{gra}{RGB}{100,100,100}
\definecolor{lgra}{RGB}{220,220,220}
\definecolor{MPG}{RGB}{000,125,122} % MPG green
\definecolor{dgr}{RGB}{000,125,122} % MPG green
\definecolor{dgre}{RGB}{000,125,122} % MPG green
\definecolor{ora}{HTML}{FF9933}

\definecolor{AMPurple}{HTML}{663366}
\definecolor{Burgundy}{HTML}{993333}
\definecolor{Coffee}{HTML}{7B6049}
\definecolor{ForestGreen}{HTML}{005826}
\definecolor{Lavender}{HTML}{6E6AB1}
\definecolor{PSLightBlue}{HTML}{7DA7D9}

\definecolor{viridis-start}{rgb}{0.96489,0.90232,0.12394}%
\definecolor{viridis-end}{rgb}{0.26700,0.00487,0.32942}%

\usepackage[setpagesize=false,
            colorlinks=true,
            linkcolor=black,
            citecolor=black,
            urlcolor=black,
            hyperfootnotes=false]{hyperref}

\usepackage{mathtools}

\usepackage{amssymb}
\usepackage[overload]{empheq} 
\usepackage{amsthm}
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{pifont}
\makeatletter
\newcommand{\repeatable}[2]{%
  \label{#1}\global\@namedef{repeatable@#1}{#2}#2
}
\newcommand{\eqrepeat}[1]{%
  \@ifundefined{repeatable@#1}{NOT FOUND}{\@nameuse{repeatable@#1}}%
  \tag{\ref{#1}}}
\makeatother

\usepackage[capitalise]{cleveref} 
\newtheorem{theorem}{Theorem}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{desideratum}[theorem]{Desideratum}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{hypothesis}[theorem]{Hypothesis}
\newtheorem{example}[theorem]{Example}


\usepackage{adjustbox}
\usepackage{epigraph}
\usepackage{amsfonts}
\usepackage{mdframed}
\usepackage{afterpage}
\usepackage{nicefrac}
\usepackage{tensor}

\newcommand{\Require}{\REQUIRE}
\newcommand{\For}{\FOR}
\newcommand{\EndFor}{\ENDFOR}
\newcommand{\If}{\IF}
\newcommand{\EndIf}{\ENDIF}
\newcommand{\State}{\STATE}
\newcommand{\Ensure}{\ENSURE}

\newcommand{\todo}[1]{\emph{\textcolor{red}{#1}}}

\usepackage{graphicx}
\usepackage{array} % used for the >{\bfseries} trick
\usepackage{booktabs} % \toprule \midrule etc.
\usepackage{multirow}
\usepackage{subcaption} % for subfigures



\usepackage{pdflscape}

% For graphs
\usepackage{tikz}
\usetikzlibrary{arrows,shapes,plotmarks}

\tikzset{>=stealth'} 
\tikzstyle{graphnode} = 
   [circle,draw=black,minimum size=22pt,text centered,text
     width=22pt,inner sep=0pt] 
\tikzstyle{var}   =[graphnode,fill=white]
\tikzstyle{obs}   =[graphnode,fill=black,text=white]
\tikzstyle{fac}   =[rectangle,draw=black,fill=black!25,minimum size=5pt]
\tikzstyle{facprior} =[rectangle,draw=black,fill=black,text=white,minimum size=5pt]
\tikzstyle{edge}  =[draw=white,double=black,thick,-]
\tikzstyle{prior} =[rectangle, draw=black, fill=black, minimum size=
5pt, inner sep=0pt]
\tikzstyle{dirprior} = [circle, draw=black, fill=black, minimum
size=5pt, inner sep=0pt]


\usepackage{pgfplots}
\pgfplotsset{compat=newest}

\pgfplotsset{
  every axis legend/.append style =
    {
      cells = { anchor = east },
      draw  = none
    },
}  
\makeatletter
\pgfplotsset{ 
    range frame/.style={
        tick align = outside,
        axis line style={opacity=0},
        after end axis/.code={
            \draw ({rel axis cs:0,0}-|{axis cs:\pgfplots@data@xmin,0}) -- ({rel axis cs:0,0}-|{axis cs:\pgfplots@data@xmax,0});
            \draw ({rel axis cs:0,0}|-{axis cs:0,\pgfplots@data@ymin}) -- ({rel axis cs:0,0}|-{axis cs:0,\pgfplots@data@ymax});
        }
    }
}
\makeatother

\pgfkeys{/pgfplots/mytuftestyle/.style={
  semithick,
  tick style={major tick length=4pt,semithick,black},
  separate axis lines,
  axis x line*=bottom,
  axis x line shift=5pt,
  xlabel shift=0pt,
  axis y line*=left,
  tick align = outside,
  axis y line shift=5pt,
  ylabel shift=0pt}}

% TIKZ
\usetikzlibrary{plotmarks}
\usepgfplotslibrary{groupplots}
\pgfplotsset{plot coordinates/math parser=false}       
\pgfkeys{/pgfplots/mystyle/.style={
  semithick,
  tick style={major tick length=4pt,semithick,gray},
  xtick align = inside,
  ytick align = inside,
  xlabel near ticks,
  ylabel near ticks,

  }}
% Check out version 30, if this trick fails ...
\newlength\figureheight
\newlength\figurewidth
\newlength\figheight
\newlength\figwidth

% For algorithms
% See 
% http://en.wikibooks.org/wiki/LaTeX/Algorithms

\usepackage{tgheros}

\usepackage{slantsc}
\usepackage{microtype}
\newcommand{\widebar}[1]{\overline{#1}}

\setcounter{secnumdepth}{3}
\setcounter{tocdepth}{1}

\usepackage{csquotes} % for the \enquote command


\usepackage{stmaryrd} % for \sslash 


\newcommand{\algalign}[3]{\raisebox{0pt}[-1pt][-1pt]{$\phantom{#1}\mathllap{#2{}}$ $\gets {}#3$}}


\definecolor{newcode}{RGB}{220,220,220}
\newcommand{\AState}[1]{\State \colorbox{newcode}{{#1}}} % additional state


\newcommand{\sign}{\operatorname{sign}}
\newcommand{\g}{\,|\,} 
\newcommand{\de}{\partial}
\renewcommand{\d}{\:d} 
\newcommand{\eps}{\epsilon}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\ddd}{\mathsf{d}}
\newcommand{\DD}{\mathsf{D}}
\newcommand{\Proba}{\mathbb{P}}
\newcommand{\proba}[1]{\Proba\left (#1\right )}% probability of an event
\newcommand{\Exp}{\mathbb{E}}
\newcommand{\Var}{\mathbb{V}}
\newcommand{\Ent}{\mathbb{H}}
\newcommand{\Cov}{\operatorname{cov}} 
\newcommand{\cov}{\operatorname{cov}} 
\newcommand{\erf}{\operatorname{erf}} 
\renewcommand{\H}{\mathcal{H}}
\newcommand{\K}{\mathcal{K}} 
\newcommand{\KL}{\text{KL}} 
\renewcommand{\Re}{\mathbb{R}}
\newcommand{\reals}{\Re}
\newcommand{\Co}{\mathbb{C}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\const}{\text{const.}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\Dcal}{\mathcal{D}} 
\newcommand{\N}{\mathcal{N}} 
\newcommand{\W}{\mathcal{W}} 
\newcommand{\cS}{\mathcal{S}} 
\newcommand{\sT}{\mathsf{T}} 
\newcommand{\B}{\mathcal{B}} 
\newcommand{\Trans}{^{\intercal}} 
\newcommand{\inv}[1]{#1^{-\!1}}
\newcommand{\iTrans}{^{-\intercal}} 
\newcommand{\argmin}{\operatorname*{arg\:min}}
\newcommand{\argmax}{\operatorname*{arg\:max}}
\renewcommand{\det}{\operatorname{det}}
\newcommand{\var}{\operatorname{var}}
\renewcommand{\=}{\operatorname*{=}}
\newcommand{\myexp}[1]{\exp{\left[ #1 \right] }}
\newcommand{\expmap}{\mathrm{Exp}}
\newcommand{\logmap}{\mathrm{Log}}
\newcommand{\spa}{\operatorname{span}}

\newcommand{\ostimes}{\circledast}

% %%% all this just to load one document from MnSymbol. See also "FindSymbol.tex".
% \DeclareFontFamily{U} {MnSymbolC}{}
% \DeclareFontShape{U}{MnSymbolC}{m}{n}{
%   <-6> MnSymbolC5
%   <6-7> MnSymbolC6
%   <7-8> MnSymbolC7
%   <8-9> MnSymbolC8
%   <9-10> MnSymbolC9
%   <10-12> MnSymbolC10
%   <12-> MnSymbolC12}{}
% \DeclareFontShape{U}{MnSymbolC}{b}{n}{
%   <-6> MnSymbolC-Bold5
%   <6-7> MnSymbolC-Bold6
%   <7-8> MnSymbolC-Bold7
%   <8-9> MnSymbolC-Bold8
%   <9-10> MnSymbolC-Bold9
%   <10-12> MnSymbolC-Bold10
%   <12-> MnSymbolC-Bold12}{}


\newcommand{\utr}{\boxbackslash}
\newcommand{\ltr}{\boxslash}
\newcommand{\oodot}{\circledcirc}

\newcommand{\hl}[1]{\textcolor{blue}{#1}}

\newcommand{\q}{\quad}
\newcommand{\qq}{\qquad}
\newcommand{\qqq}{\quad\qquad}
\newcommand{\qqqq}{\qquad\qquad}

\renewcommand{\vec}{\boldsymbol} 
\newcommand{\mat}{\boldsymbol} 
\newcommand{\vect}[1]{\overrightarrow{#1}}
\newcommand{\vest}[1]{\overrightharpoon{#1}}
\newcommand{\fun}[1]{\mathsf{#1}}
\newcommand{\logm}{\operatorname{Log}}
\newcommand{\expm}{\operatorname{Exp}}
\renewcommand{\O}{\mathcal{O}} 
\newcommand{\GP}{\mathcal{GP}}
\newcommand{\Id}{\vec{I}}
\newcommand{\zero}{\vec{0}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\rk}{\operatorname{rk}}
\newcommand{\II}{\mathbb{I}}
\renewcommand{\L}{\mathcal{L}}

\newcommand{\bm}{\boldsymbol{m}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\GramMat}{\mat G}

\newcommand{\w}{\vec{w}}
\newcommand{\f}{\vec{f}}
\newcommand{\y}{\vec{y}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\X}{\mathbb{X}}

\newcommand{\fS}{\mathsf{S}}
\newcommand{\fW}{\mathsf{W}}
\newcommand{\fB}{\mathsf{B}}
\newcommand{\fK}{\mathsf{K}}
\newcommand{\fH}{\mathsf{H}}
\newcommand{\fk}{\mathsf{k}}
\newcommand{\fh}{\mathsf{h}}
\newcommand{\fL}{\mathsf{L}}

\newcommand{\sA}{\boldsymbol{\mathsf{A}}}
\newcommand{\sB}{\boldsymbol{\mathsf{B}}}
\newcommand{\sC}{\boldsymbol{\mathsf{C}}}

\usepackage{colonequals}
\newcommand{\ce}{\colonequals}
\newcommand{\ec}{\equalscolon}

\newcommand{\braket}[2]{\left\langle #1 , #2 \right\rangle}
\newcommand{\brakets}[3]{\left\langle #1 \, \middle| \, #2 \, \middle|\, #3 \right\rangle}

\usetikzlibrary{arrows,shapes,plotmarks}

\tikzset{>=stealth'} 
\tikzstyle{graphnode} = 
   [circle,draw=black,minimum size=22pt,text centered,text
     width=22pt,inner sep=0pt] 
\tikzstyle{var}   =[graphnode,fill=white]
\tikzstyle{obs}   =[graphnode,fill=black,text=white]
\tikzstyle{fac}   =[rectangle,draw=black,fill=black!25,minimum size=5pt]
\tikzstyle{facprior} =[rectangle,draw=black,fill=black,text=white,minimum size=5pt]
\tikzstyle{edge}  =[draw=white,double=black,thick,-]
\tikzstyle{prior} =[rectangle, draw=black, fill=black, minimum size=
5pt, inner sep=0pt]
\tikzstyle{dirprior} = [circle, draw=black, fill=black, minimum
size=5pt, inner sep=0pt]

% to avoid warnings, copy only two symbols from stmaryrd
\DeclareSymbolFont{stmry}{U}{stmry}{m}{n}
\DeclareMathSymbol\leftarrowtriangle\mathrel{stmry}{"5E}
\DeclareMathSymbol\rightarrowtriangle\mathrel{stmry}{"5F}
\renewcommand{\gets}{\operatorname*{\leftarrowtriangle}}
\renewcommand{\to}{\operatorname*{\rightarrowtriangle}}

\usepackage{tensor}
% Left and right kernel derivatives
\newcommand{\dk}{\tensor[^{\de}]{k}{}}
\newcommand{\ddk}{\tensor[^{\de^2}]{k}{}}
\newcommand{\ddkd}{\tensor[^{\de^2}]{k}{^{\de}}}
\newcommand{\dddk}{\tensor[^{\de^3}]{k}{}}
\newcommand{\dddkd}{\tensor[^{\de^3}]{k}{^{\de}}}
\newcommand{\kd}{\tensor{k}{^{\de}}}
\newcommand{\dkd}{\tensor[^{\de}]{k}{^{\de}}}

\newcommand{\dy}{y^{\de}}


\newcommand{\indM}[2]{{[#1]}_{#2}}
\newcommand{\eqcomment}[1]{\\&\sslash\text{{\small\emph{#1}}}\notag}
\newcommand{\reqcomment}[1]{\\&\sslash\text{\textcolor{blue}{{\small\emph{#1}}}\notag}}

\newcommand{\pname}[1]{\emph{#1}} % style for proper names
\newcommand{\latin}[1]{\emph{#1}} % style for latin phrases
\newcommand{\adhoc}{\latin{ad hoc}}
\newcommand{\ie}{\latin{i.e.~}}
\newcommand{\eg}{\latin{e.g.~}}
\newcommand{\cf}{\latin{c.f.~}}
\newcommand{\etc}{\latin{etc.~}}

% Kronecker symbols
\makeatletter
\newcommand{\superimpose}[2]{%s
  {\ooalign{$#1\@firstoftwo#2$\cr\hfil$#1\@secondoftwo#2$\hfil\cr}}}
\makeatother
\newcommand{\sk}{\mathpalette\superimpose{{\otimes}{\ominus}}}
\newcommand{\kr}{\otimes}
\newcommand{\vecm}[1]{\operatorname{vec}\left(#1\right)} % vectorized matrix
\newcommand{\vecmtrans}[1]{\vecm{#1}\Trans} % vectorized matrix transposed (i.e. the vector -- not the matrix)
\newcommand{\tomat}[1]{\operatorname{mat}\left(#1\right)} % transform vector to matrix

\newcommand{\integr}[1][\ ]{\int\limits_{#1} \! }
\newcommand{\dx}[1]{\ \mathrm{d}#1}

\newcommand{\deriv}[2]{\frac{\partial #1}{\partial #2}}

\newcommand{\stack}[2]{\begin{bmatrix}
#1 \\ #2
\end{bmatrix}}
\newcommand{\concat}[2]{\begin{bmatrix}
#1 & #2
\end{bmatrix}}

\newcommand{\A}{\mat A} % A
\newcommand{\Ai}{\A^{-\!1}} % symbol for A inverse
\renewcommand{\b}{\vec b} % b
\newcommand{\x}{\vec{x}^\ast}

% commands for estimation of determinants
\renewcommand{\l}[1]{l_{#1}} %
\newcommand{\abs}{\operatorname{abs}} % absolute value (to distuingish from the determinant)

\newcommand{\SP}{S} % the number of stopping points
\newcommand{\me}[1][\tau]{\hat{\mu}_{#1}} % population mean estimate
\newcommand{\est}[1][\tau]{(N-#1)\me[#1]} % estimator actually used
\newcommand{\tme}{\tilde{\mu}_\tau(m)} % mean estimate of iid variables
\newcommand{\ve}{\hat{\sigma^2}_\tau(m)} % population variance estimate
\newcommand{\tve}{\tilde{\sigma^2}_\tau(m)} % variance estimate of iid variables
\newcommand{\tstart}{t} % The time we start to calculate our empirical values.
\newcommand{\lBound}{C} % upper bound for \l{}_j-\Exp[\tilde{}_j\mid x_1, ..., x_{j-1}]
\newcommand{\Dhat}{\hat{D}_N} % the estimator for the log-determinant

\newcommand{\kj}[1][j]{\vec k_{#1}(\vec x)} % k_j(x) = [k(x, x_1), ..., k(x, x_j)]\Trans
\newcommand{\kjx}[2]{\vec k_{#1}(\vec #2)} % k_j(x) = [k(x, x_1), ..., k(x, x_j)]\Trans

\renewcommand{\L}{\mathcal{L}}

\newcommand{\stopTimeOne}{\sign(\U_n)=\sign(\L_n)\neq 0}
\newcommand{\stopTimeTwo}{\frac{\U_n-\L_n}{2\min(\abs(\U_n), \abs(\L_n))} \leq r}



% % from the STCO paper
\newcommand{\set}[1]{\{#1\}}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\inner}[1]{\langle #1 \rangle}


% CoRel notation
\newcommand{\factorP}{\mathbb{P}_f}
\newcommand{\bo}{BO}
\newcommand{\CoRel}{CoRel}
\newcommand{\GFP}{GFP}
\newcommand{\RFP}{RFP}

\newcommand{\simon}[1]{\textcolor{dred}{\textbf{#1}}}
\newcommand{\richard}[1]{\textcolor{dblu}{\textbf{#1}}}
